Beyond Theorems: A Counterexample to Potential Markov Game Criteria

There are only limited classes of multi-player stochastic games in which independent learning is guaranteed to converge to a Nash equilibrium. Markov potential games are a key example of such classes. Prior work has outlined sets of sufficient conditions for a stochastic game to qualify as a Markov potential game. However, these conditions often impose strict limitations on the game's structure and tend to be challenging to verify. To address these limitations, Mguni et al. [12] introduce a relaxed notion of Markov potential games and offer an alternative set of necessary conditions for categorizing stochastic games as potential games. Under these conditions, the authors claim that a deterministic Nash equilibrium can be computed efficiently by solving a dual Markov decision process. In this paper, we offer evidence refuting this claim by presenting a counterexample.

==> Sections/4-exp.tex <==
\subsection{Independent-learning Dynamics}
For MPGs, independently policy gradient in the form of projected stochastic gradient ascent (PSGA) converges to an $\epsilon$-Nash equilibrium at a rate of $O(1/\epsilon^2)$~\cite{leonardos2021global}. PSGA is a variant of projected gradient ascent (PGA) in which the actual gradient is replaced by an estimate that is calculated from a randomly selected sample of trajectories.
With batch size $T$, the estimate of the gradient of agent $i$'s value function at iteration $t$ is modeled as:
\[
 \hat{\nabla}_{\pi_i}^{(t)}=R_i^{(T,t)}\sum_{k=0}^{T} \nabla \log(\pi_i(a_{i,k}^{(t)}|s_k^{(t)})),
\]
where $R_i^{(T,t)}=\sum_{k=0}^{T} r_{i,t}^k$. 
Therefore, with learning rate $\eta$, the policy update for each agent $i$ is modeled as:
\[
 \pi_i^{(t+1)} \coloneqq P_{\Delta(A_i)^S}(\pi_i^{(t)} + \eta \hat{\nabla}_{\pi_i}^{(t)}),
\]
where $P_{\Delta(A_i)^S}$ is the Euclidean projection onto $\Delta(A_i)^S$.
In this section, we present experimental results for deploying deep deterministic policy gradient (DDPG)~\cite{lillicrap2015continuous}. We parametrize each agent's strategy and use deep learning to update parameters. Because DDPG uses neural networks to estimate strategy and value function, it is suitable for our setting in which both action and state spaces are continuous.
% Since action spaces and the state space are continuous, we use a Gaussian distribution to represent each agent's strategy~\cite{sutton2018reinforcement, van2007reinforcement}:
% \[
%  \pi_i(a_i \given s, \theta_i) = \frac{1}{\sigma(s, \theta_i^{\sigma})\sqrt{2\pi}} \exp(-\frac{(a_i-\mu(s, \theta_i^{\mu}))^2}{2\sigma(s, \theta_i^{\sigma})^2}),
% \]
% where $\theta_i = (\theta_i^\sigma, \theta_i^\mu)$ represents agent $i$'s strategy parameters.
% We use linear function approximation to model $\sigma(s, \theta_i^{\sigma})$ and $\mu(s, \theta_i^\mu)$.
% In our experiments, for stochastic gradient updates, we use mini batches of size 100.

\reffig{fig:combined} show our experimental results for deploying DDPG to our counterexample.
As expected, the learning dynamics do not converge to any Nash equilibrium.
This is expected as the game in our counterexample is not an MPG, and independent learning in a general stochastic games is not guaranteed to converge.

% \begin{figure}
%  \centering
%  \begin{tikzpicture}
%   \begin{axis}[
%    width=0.85\linewidth,
%    height=0.65\linewidth,
%    xlabel={Iteration},
%    ylabel={Payoff},
%    xtick={0, 750, 1500, 2250,3000},
%    xticklabels={0, 5k, 10k, 15k, 20k},
%    xmin=0, 
%    xmax=3000,
%    grid=both,
%    legend style={at={(0.64,0.55)},anchor=west,draw=black,fill=white}, nodes={scale=0.75, transform shape}
%   ]
%    \addplot[blue, smooth] table {reward1.txt};
%    \addlegendentry{Agent 1}
%    \addplot[red, smooth] table {reward2.txt};
%    \addlegendentry{Agent 2}
%   \end{axis}
%  \end{tikzpicture}
%  \caption{\textbf{MARL in the counterexample.} Players' payoffs do not converge.}
%  \label{fig:reward}
% \end{figure}

% \begin{figure}
%  \centering
%  \begin{tikzpicture}
%   \begin{axis}[
%    width=0.85\linewidth,
%    height=0.65\linewidth,
%    xlabel={Iteration},
%    ylabel={Action},
%    xtick={0, 750, 1500, 2250,3000},
%    xticklabels={0, 5k, 10k, 15k, 20k},
%    xmin=0, 
%    xmax=3000,
%    grid=both,
%    legend style={at={(0.64,0.55)},anchor=west,draw=black,fill=white},nodes={scale=0.75, transform shape}
%   ]
%    \addplot[blue, smooth] table {action1.txt};
%    \addlegendentry{Agent 1}
%    \addplot[red, smooth] table {action2.txt};
%    \addlegendentry{Agent 2}
%   \end{axis}
%  \end{tikzpicture}
%  \caption{\textbf{MARL in the counterexample.} Players' actions do not converge.}
%  \label{fig:action}
% \end{figure}


% \usepackage{pgfplots}
\definecolor{customcolor1}{HTML}{491F40} %dark purple
% \definecolor{customcolor1}{HTML}{457373}
% \definecolor{customcolor2}{HTML}{003049} % dark blue
\definecolor{customcolor2}{HTML}{D6866B}
% \definecolor{customcolor1}{HTML}{DBA79C}


% \definecolor{customcolor2}{HTML}{CD7E59}



\begin{figure}
 \centering
 \begin{minipage}{0.48\textwidth}
 \begin{tikzpicture}
  \begin{axis}[
   width=0.9\linewidth,
   height=0.65\linewidth,
   xlabel={Iteration},
   ylabel={Payoff},
   xtick={0, 750, 1500, 2250,3000},
   xticklabels={0, 5k, 10k, 15k, 20k},
   xmin=0, 
   xmax=3000,
   grid=both,
   legend style={at={(0.64,0.55)},anchor=west,draw=black,fill=white}, nodes={scale=0.75, transform shape}
  ]
   \addplot[customcolor2, smooth] table {reward1.txt};
   \addlegendentry{Agent 1}
   \addplot[customcolor1, smooth] table {reward2.txt};
   \addlegendentry{Agent 2}
  \end{axis}
 \end{tikzpicture}
 \end{minipage}
 \hfill
 \begin{minipage}{0.48\textwidth}
 \begin{tikzpicture}
  \begin{axis}[
   width=0.9\linewidth,
   height=0.65\linewidth,
   xlabel={Iteration},
   ylabel={Action},
   xtick={0, 750, 1500, 2250,3000},
   xticklabels={0, 5k, 10k, 15k, 20k},
   xmin=0, 
   xmax=3000,
   grid=both,
   legend style={at={(0.64,0.55)},anchor=west,draw=black,fill=white}, nodes={scale=0.75, transform shape}
  ]
   \addplot[customcolor2, smooth] table {action1.txt};
   \addlegendentry{Agent 1}
   \addplot[customcolor1, smooth] table {action2.txt};
   \addlegendentry{Agent 2}
  \end{axis}
 \end{tikzpicture}
 \end{minipage}
 \small\caption{\textbf{MARL in the counterexample.} Top: Players' payoffs and actions do not converge to any equilibrium.}
 \label{fig:combined}
\end{figure}



==> Sections/5-solution.tex <==
\section{Alternative Condition}
\label{sec:cst}
In this section, we provide a new condition and prove that it ensures that \refclm{clm:opsp-mpg} always holds under some standard assumptions.
In the rest of this section, we first state our assumptions.
We then formally provide our new condition.
Finally, we prove that our new condition ensure that \refclm{clm:opsp-mpg} always holds.

\subsection{Assumptions}\label{subsec:assumptions}
Our results in this section are built under the following assumptions:
\begin{itemize}[leftmargin=*,noitemsep=*,topsep=1pt]
    \item \textbf{Asm.\ 1.} The payoff functions are bounded and measurable in action inputs.
    \item \textbf{Asm.\ 2.} The payoff functions are Lipschitz continuous.
    \item \textbf{Asm.\ 3.} The payoff functions are continuously differentiable in the state and action inputs. % we need this to show that phi is bounded.
%    \item \textbf{Assumption 4.} Strategies are differentiable with respect to the strategy parameters. 
\end{itemize}
We are now ready to formally introduce our new condition.

\subsection{Complete State Transitivity}
We now introduce our new condition called the \emph{complete state transitivity}:
\begin{condition}[\textbf{Complete state transitivity}]
\label{con:cst}
 An OPSG with potential function $\Phi$ satisfies complete state transitivity if for all agents $i \in N$, we have:
 \begin{align*}
  \int_{\bm{a} \in \bm{A}} r_i(s,\bm{a}) \bm{\pi}(\bm{a} \given s) d\bm{a} - \int_{\bm{a} \in \bm{A}} r_i(s^\prime,\bm{a}) \bm{\pi}(\bm{a} \given s^\prime) d\bm{a} =\\
  \int_{\bm{a} \in \bm{A}} \Phi(s,\bm{a}) \bm{\pi}(\bm{a} \given s) d\bm{a} - \int_{\bm{a} \in \bm{A}} \Phi(s^\prime,\bm{a}) \bm{\pi}(\bm{a} \given s^\prime) d\bm{a},
 \end{align*}
 for all states $s, s^\prime \in S$, and all joint strategy profiles $\bm{\pi} \in \bm{\Pi}$.
\end{condition}
\noindent
Compared to state transitivity which concerns immediate payoffs, complete state transitivity puts restrictions on expected immediate payoffs.
Complete state transitivity requires that the difference in expected immediate payoffs for changing state is the same for each agent.

\subsection{From omplete state transitivity to MPG}\label{subsec:from-omplete-state-transitivity-to-mpg}
We are now ready to provide our main technical result showing that $G$ has a deterministic stationary Nash equilibrium that can be efficiently computed by solving $G$'s dual MDP\@.

\begin{prop}
\label{prop:v-phi-diff}
 Let $G$ be an $n$-agent OPSG with one-shot potential function $\Phi$ that satisfies complete state transitivity.
 For all agents $i \in N$ and strategies $\bm{\pi} \in \bm{\Pi}$, let $V_i^{\bm{\pi}}(\cdot)$ be defined according to \refequ{eq:value}.
 Define $B^{\bm{\pi}}$ for any strategy $\bm{\pi} \in \bm{\Pi}$ as:
 \begin{equation}
 \label{eq:B}
  B^{\bm{\pi}}(s) \triangleq \EE_{\bm{\pi}} \left[ \sum_{t=0}^{\infty} \gamma^t \Phi(s_t, \bm{a_t}) \given[\Big] s_0 = s \right].
 \end{equation}
 Then we have:
 \begin{equation}
 \label{eq:v-phi-diff}
  V_i^{\bm{\pi}}(s) - V_i^{(\pi^\prime, \bm{\pi_{-i}})}(s) = B^{\bm{\pi}}(s) - B^{(\pi^\prime, \bm{\pi_{-i}})}(s)
 \end{equation}
 for all agents $i \in N$, all states $s \in S$, all joint strategies $\bm{\pi} = (\pi_i, \bm{\pi}_{-i}) \in \bm{\Pi}$, and all strategies $\pi_i^\prime \in \Pi_i$.
\end{prop}
\noindent
We prove the proposition in two steps.
We first start with the finite-horizon case, and then we extend the proof to the infinite-horizon case.

\subsection{Finite-horizon Case}\label{subsec:finite-horizon-case}

Suppose that $G$ is a finite-horizon game of length $T \in \NN$.
For all agents $i$, any joint strategy $\bm{\pi} \in \bm{\Phi}$, and any $0< k \le T$, let us define $V_{k, i}^{T,\bm{\pi}}(s)$ as:
\begin{equation*}
 V_{k, i}^{T,\bm{\pi}}(s) \triangleq \EE_{\bm{\pi}} \left[ \sum_{t=0}^{T-k} \gamma^t r_i(s_t, \bm{a_t}) \given  s_0 = s \right].
\end{equation*}
We further define $B_k^{T,\bm{\pi}}(s)$ for any joint strategy $\bm{\pi} \in \bm{\Phi}$:
\begin{equation*}
 B_k^{T,\bm{\pi}}(s) \triangleq \EE_{\bm{\pi}} \left[ \sum_{t=0}^{T-k} \gamma^t \Phi(s_t, \bm{a_t}) \given[\Big] s_0 = s \right].
\end{equation*}
We seek to show the following:
\[
 V_{1,i}^{T,\bm{\pi}}(s) - V_{1,i}^{T, (\pi^\prime, \bm{\pi_{-i}})}(s) = B_1^{T, \bm{\pi}}(s) - B_1^{T, (\pi^\prime, \bm{\pi_{-i}})}(s)
\]
for all agents $i \in N$, all states $s \in S$, all joint strategies $\bm{\pi} = (\pi_i, \bm{\pi}_{-i}) \in \bm{\Pi}$, and all strategies $\pi_i^\prime \in \Pi_i$.
Our proof is by induction on $k$.
We prove the following two inductive expressions for $1 \le k \le T$:
\[
 V_{k, i}^{T,\bm{\pi}}(s) - V_{k, i}^{T,(\pi_i^\prime,\bm{\pi_{-i}})}(s) = B_{k}^{T,\bm{\pi}}(s) - B_{k}^{T,(\pi_i^\prime,\bm{\pi_{-i}})}(s),
\]
and
\[
 V_{k, i}^{T,\bm{\pi}}(s) - V_{k, i}^{T,\bm{\pi}}(s^\prime) = B_{k}^{T,\bm{\pi}}(s) - B_{k}^{T,\bm{\pi}}(s^\prime).
\]
 
\begin{proof}
 Consider the base case of $k = T$.
 We start with the first inductive expression.
 For all agents $i \in N$, all states $s \in S$, any joint strategy $\bm{\pi} = (\pi_i, \bm{\pi_{-i}}) \in \bm{\Pi}$, any strategy $\pi_i^\prime \in \Pi_i$, and any $a_i^\prime \in A_i$, we have:
 \begin{align}
  \label{eq:ind-T-1}
  \ifthenelse{\boolean{arxiv}}{
   V_{T, i}^{T,\bm{\pi}}(s) - B_{T}^{T,\bm{\pi}}(s) &= \int_{a_i}\pi_i(a_i \given s) \EE_{\bm{\pi_{-i}}(s)} [r_i(s,a_i,\bm{a_{-i}}) - \Phi(s,a_i,\bm{a_{-i}}) ] da_i \nonumber \\
   &=\int_{a_i}\pi_i(a_i \given s) \EE_{\bm{\pi_{-i}}(s)} [r_i(s,a_i^\prime,\bm{a_{-i}})- \Phi(s,a_i^\prime,\bm{a_{-i}}) ] da_i \nonumber \\
   &=\int_{a_i}\pi_i(a_i \given s)da_i \EE_{\bm{\pi_{-i}}(s)} [r_i(s,a_i^\prime,\bm{a_{-i}}) - \Phi(s,a_i^\prime,\bm{a_{-i}}) ] \nonumber \\
   &=\int_{a_i}\pi_i^\prime(a_i \given s)da_i \EE_{\bm{\pi_{-i}}(s)} [r_i(s,a_i^\prime,\bm{a_{-i}}) - \Phi(s,a_i^\prime,\bm{a_{-i}}) ] \nonumber \\
   &=\int_{a_i}\pi_i^\prime(a_i \given s) \EE_{\bm{\pi_{-i}}(s)} [r_i(s,a_i,\bm{a_{-i}}) - \Phi(s,a_i,\bm{a_{-i}}) ] da_i \nonumber \\[0.65em]
   &=V_{T, i}^{T,(\pi_i^\prime,\bm{\pi_{-i}})}(s) - B_{T}^{T,(\pi_i^\prime,\bm{\pi_{-i}})}(s),
  }{
   &V_{T, i}^{T,\bm{\pi}}(s) - B_{T}^{T,\bm{\pi}}(s) = \nonumber \\
   &\int_{a_i}\pi_i(a_i \given s) \EE_{\bm{\pi_{-i}}(s)} [r_i(s,a_i,\bm{a_{-i}}) - \Phi(s,a_i,\bm{a_{-i}}) ] da_i = \nonumber \\
   &\int_{a_i}\pi_i(a_i \given s) \EE_{\bm{\pi_{-i}}(s)} [r_i(s,a_i^\prime,\bm{a_{-i}})- \Phi(s,a_i^\prime,\bm{a_{-i}}) ] da_i = \nonumber \\
   &\int_{a_i}\pi_i(a_i \given s)da_i \EE_{\bm{\pi_{-i}}(s)} [r_i(s,a_i^\prime,\bm{a_{-i}}) - \Phi(s,a_i^\prime,\bm{a_{-i}}) ] = \nonumber \\
   &\int_{a_i}\pi_i^\prime(a_i \given s)da_i \EE_{\bm{\pi_{-i}}(s)} [r_i(s,a_i^\prime,\bm{a_{-i}}) - \Phi(s,a_i^\prime,\bm{a_{-i}}) ] = \nonumber \\
   &\int_{a_i}\pi_i^\prime(a_i \given s) \EE_{\bm{\pi_{-i}}(s)} [r_i(s,a_i,\bm{a_{-i}}) - \Phi(s,a_i,\bm{a_{-i}}) ] da_i = \nonumber \\[0.65em]
   &V_{T, i}^{T,(\pi_i^\prime,\bm{\pi_{-i}})}(s) - B_{T}^{T,(\pi_i^\prime,\bm{\pi_{-i}})}(s),
  }
 \end{align}
 where the second equality follows from \refdef{def:one-shot}, the third one follows from the fact that the inner expectation does not depend on $a_i$, and the fifth one follows from \refdef{def:one-shot}.
 
 Next, we focus on the second inductive expression.
 For all agents $i \in N$, all states $s, s^\prime \in S$, and any joint strategy $\bm{\pi} \in \bm{\Pi}$, we have:
 \begin{align}
 \label{eq:ind-T-2}
  \ifthenelse{\boolean{arxiv}}{
   V_{T, i}^{T,\bm{\pi}}(s) - B_{T}^{T,\bm{\pi}}(s) &= \int_{\bm{a}} \bm{\pi}(\bm{a} \given s) ( r_i(s, \bm{a}) - \Phi(s, \bm{a}) ) d\bm{a} \nonumber \\
   &= \int_{\bm{a}} \bm{\pi}(\bm{a} \given s^\prime) ( r_i(s^\prime, \bm{a}) - \Phi(s^\prime, \bm{a}) ) d\bm{a} \nonumber \\[0.65em]
   &= V_{T, i}^{T,\bm{\pi}}(s^\prime) - B_{T}^{T,\bm{\pi}}(s^\prime),
  }{
   V_{T, i}^{T,\bm{\pi}}(s) &- B_{T}^{T,\bm{\pi}}(s) = \int_{\bm{a}} \bm{\pi}(\bm{a} \given s) ( r_i(s, \bm{a}) - \Phi(s, \bm{a}) ) d\bm{a} \nonumber \\
   &= \int_{\bm{a}} \bm{\pi}(\bm{a} \given s^\prime) ( r_i(s^\prime, \bm{a}) - \Phi(s^\prime, \bm{a}) ) d\bm{a} \nonumber \\[0.65em]
   &= V_{T, i}^{T,\bm{\pi}}(s^\prime) - B_{T}^{T,\bm{\pi}}(s^\prime),
  }
 \end{align}
 where the second equality holds because of \refcon{con:cst}.
 
 Next, we show that the inductive expressions hold for any $1 \le k < T$ if it holds for $k+1$.
 First, note that for any $1 \le k < T$, any state $s$, and any joint strategy $\bm{\pi}\in \bm{\Pi}$, we have:
 \begin{equation*}
  B_k^{T,\bm{\pi}}(s) = \EE_{\bm{\pi}(s)} \left[ \Phi(s, \bm{a}) + \gamma \int_{s^\prime} p(s^\prime,s,\bm{a}) B_{k+1}^{T,\bm{\pi}}(s^\prime) ds^\prime \right],
 \end{equation*}
 and, for all agents $i$, we have:
 \begin{equation*}
  V_{k,i}^{T,\bm{\pi}}(s) = \EE_{\bm{\pi}(s)} \left[ r(s, \bm{a}) + \gamma \int_{s^\prime} p(s^\prime,s,\bm{a}) V_{k+1,i}^{T,\bm{\pi}}(s^\prime) ds^\prime \right].
 \end{equation*}
 Therefore, for all agents $i \in N$, all states $s \in S$, any joint strategy $\bm{\pi} = (\pi_i, \bm{\pi_{-i}}) \in \bm{\Pi}$, any strategy $\pi_i^\prime \in \Pi_i$, and any action $a_i^\prime \in A_i$, we have the following equality:
 \begin{align}
 \label{eq:induction}
  \ifthenelse{\boolean{arxiv}}{
   V_{k, i}^{T,\bm{\pi}}(s) - B_{k}^{T,\bm{\pi}}(s) = &\EE_{\bm{\pi}(s)} [ r_i(s, \bm{a_{k}}) - \Phi(s, \bm{a_{k}}) ] \\
   &\quad +\gamma \EE_{\bm{\pi}(s)} \left[ \int_{s^\prime} p(s^\prime,s,\bm{a_k}) (V_{k+1,i}^{T,\bm{\pi}}(s^\prime) - B_{k+1}^{T,\bm{\pi}}(s^\prime)) ds^\prime \right]. \nonumber
  }{
   &V_{k, i}^{T,\bm{\pi}}(s) - B_{k}^{T,\bm{\pi}}(s) = \EE_{\bm{\pi}(s)} [ r_i(s, \bm{a_{k}}) - \Phi(s, \bm{a_{k}}) ] \\
   &\quad +\gamma \EE_{\bm{\pi}(s)} \left[ \int_{s^\prime} p(s^\prime,s,\bm{a_k}) (V_{k+1,i}^{T,\bm{\pi}}(s^\prime) - B_{k+1}^{T,\bm{\pi}}(s^\prime)) ds^\prime \right]. \nonumber
  }
 \end{align} 
 
 We now start with the first inductive expression.
 Using the same algebra as in \refequ{eq:ind-T-1}, for all agents $i \in N$, all states $s \in S$, any joint strategy $\bm{\pi} = (\pi_i, \bm{\pi_{-i}}) \in \bm{\Pi}$, and any strategy $\pi_i^\prime \in \Pi_i$, we have:
 \begin{align}
  \label{eq:ind-first}
  \ifthenelse{\boolean{arxiv}}{
   \EE_{\bm{\pi}(s)} [r_i(s,\bm{a_{k}}) - \Phi(s,\bm{a_{k}}) ]  = \EE_{(\pi_i^\prime,\bm{\pi_{-i}})(s)} [r_i(s,\bm{a_{k}}) - \Phi(s,\bm{a_{k}}) ].
  }{
   &\EE_{\bm{\pi}(s)} [r_i(s,\bm{a_{k}}) - \Phi(s,\bm{a_{k}}) ]  = \nonumber \\
   &\EE_{(\pi_i^\prime,\bm{\pi_{-i}})(s)} [r_i(s,\bm{a_{k}}) - \Phi(s,\bm{a_{k}}) ].
  }
 \end{align}
 On the other hand, we have:
 \begin{align}
 \label{eq:ind-second}
  \ifthenelse{\boolean{arxiv}}{
   \EE_{\bm{\pi}(s)} \left[ \int_{s^\prime} p(s^\prime,s,\bm{a_k}) (V_{k+1,i}^{T,\bm{\pi}}(s^\prime) - B_{k+1}^{T,\bm{\pi}}(s^\prime)) ds^\prime \right] &= \EE_{\bm{\pi}(s)} \left[ \int_{s^\prime} p(s^\prime,s,\bm{a_k}) (V_{k+1,i}^{T,\bm{\pi}}(s) - B_{k+1}^{T,\bm{\pi}}(s)) ds^\prime \right] \nonumber \\
   &=\EE_{\bm{\pi}(s)} \left[ (V_{k+1,i}^{T,\bm{\pi}}(s) - B_{k+1}^{T,\bm{\pi}}(s)) \int_{s^\prime} p(s^\prime,s,\bm{a_k}) ds^\prime \right] \nonumber \\
   &=\EE_{\bm{\pi}(s)} \left[ V_{k+1,i}^{T,\bm{\pi}}(s) - B_{k+1}^{T,\bm{\pi}}(s) \right] \nonumber \\
   &=V_{k+1,i}^{T,\bm{\pi}}(s) - B_{k+1}^{T,\bm{\pi}}(s),
  }{
   &\EE_{\bm{\pi}(s)} \left[ \int_{s^\prime} p(s^\prime,s,\bm{a_k}) (V_{k+1,i}^{T,\bm{\pi}}(s^\prime) - B_{k+1}^{T,\bm{\pi}}(s^\prime)) ds^\prime \right] = \nonumber \\
   &\EE_{\bm{\pi}(s)} \left[ \int_{s^\prime} p(s^\prime,s,\bm{a_k}) (V_{k+1,i}^{T,\bm{\pi}}(s) - B_{k+1}^{T,\bm{\pi}}(s)) ds^\prime \right] = \nonumber \\
   &\EE_{\bm{\pi}(s)} \left[ (V_{k+1,i}^{T,\bm{\pi}}(s) - B_{k+1}^{T,\bm{\pi}}(s)) \int_{s^\prime} p(s^\prime,s,\bm{a_k}) ds^\prime \right] = \nonumber \\
   &\EE_{\bm{\pi}(s)} \left[ V_{k+1,i}^{T,\bm{\pi}}(s) - B_{k+1}^{T,\bm{\pi}}(s) \right] = \nonumber \\
   &V_{k+1,i}^{T,\bm{\pi}}(s) - B_{k+1}^{T,\bm{\pi}}(s),
  }
 \end{align}
 where the first equality follows from the inductive assumption (\refequ{eq:ind-T-2} holds for $k+1$), and the forth equality follows from the fact that $V_{k+1,i}$ and $B_{k+1}$ do not depend on the action taken at step $k$.
 By the inductive assumption (\refequ{eq:ind-T-1} holds for $k+1$), we have:
 \[
  V_{k+1,i}^{T,\bm{\pi}}(s) - B_{k+1}^{T,\bm{\pi}}(s) = V_{k+1,i}^{T,(\pi_i^\prime,\bm{\pi_{-i}})}(s) - B_{k+1}^{T,(\pi_i^\prime,\bm{\pi_{-i}})}(s).
 \]
 Applying \refequ{eq:ind-second} again to $V_{k+1,i}^{T,(\pi_i^\prime,\bm{\pi_{-i}})}(s) - B_{k+1}^{T,(\pi_i^\prime,\bm{\pi_{-i}})}(s)$, we have:
 \begin{align}
  \label{eq:ind-third}
  \ifthenelse{\boolean{arxiv}}{
   V_{k+1,i}^{T,(\pi_i^\prime,\bm{\pi_{-i}})}(s) &- B_{k+1}^{T,(\pi_i^\prime,\bm{\pi_{-i}})}(s) = \\
   &\EE_{(\pi_i^\prime,\bm{\pi_{-i}})(s)} \left[ \int_{s^\prime} p(s^\prime,s,\bm{a_k}) (V_{k+1,i}^{T,(\pi_i^\prime,\bm{\pi_{-i}})}(s^\prime) - B_{k+1}^{T,(\pi_i^\prime,\bm{\pi_{-i}})}(s^\prime)) ds^\prime \right].\nonumber
  }{
   &V_{k+1,i}^{T,(\pi_i^\prime,\bm{\pi_{-i}})}(s) - B_{k+1}^{T,(\pi_i^\prime,\bm{\pi_{-i}})}(s) = \\
   &\EE_{(\pi_i^\prime,\bm{\pi_{-i}})(s)} \bigg[ \int_{s^\prime} p(s^\prime,s,\bm{a_k}) (V_{k+1,i}^{T,(\pi_i^\prime,\bm{\pi_{-i}})}(s^\prime) \nonumber \\
   &\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad - B_{k+1}^{T,(\pi_i^\prime,\bm{\pi_{-i}})}(s^\prime)) ds^\prime \bigg] \nonumber.
  }
 \end{align}
 Substituting \refequ{eq:ind-first} and \refequ{eq:ind-third} in \refequ{eq:induction}, we get:
 \[
  V_{k, i}^{T,\bm{\pi}}(s) - B_{k}^{T,\bm{\pi}}(s) = V_{k, i}^{T,\bm{\pi^\prime}}(s) - B_{k}^{T,\bm{\pi^\prime}}(s).
 \]
 
 We now focus on the second inductive expression.
 For all agents $i \in N$, all states $s, s^\prime \in S$, any joint strategy $\bm{\pi} \in \bm{\Pi}$, \refcon{con:cst} implies the following:
 \begin{align}
  \label{eq:second-ind-1}
  \ifthenelse{\boolean{arxiv}}{
   \EE_{\bm{\pi}(\cdot,s)} [ r_i(s, \bm{a_{k}}) - \Phi(s, \bm{a_{k}}) ] = \EE_{\bm{\pi}(\cdot,s^\prime)} [ r_i(s^\prime, \bm{a_{k}}) - \Phi(s^\prime, \bm{a_{k}}) ].
  }{
   &\EE_{\bm{\pi}(\cdot,s)} [ r_i(s, \bm{a_{k}}) - \Phi(s, \bm{a_{k}}) ] = \\
   &\EE_{\bm{\pi}(\cdot,s^\prime)} [ r_i(s^\prime, \bm{a_{k}}) - \Phi(s^\prime, \bm{a_{k}}) ]. \nonumber
  }
 \end{align}
 Moreover, for all agents $i \in N$, all states $s, s^\prime \in S$, and any joint strategy $\bm{\pi} \in \bm{\Pi}$, we have:
 \begin{align}
  \label{eq:second-ind-2}
  \ifthenelse{\boolean{arxiv}}{
   V_{k+1, i}^{T,\bm{\pi}}(s) - B_{k+1}^{T,\bm{\pi}}(s) &= V_{k+1, i}^{T,\bm{\pi}}(s^\prime) - B_{k+1}^{T,\bm{\pi}}(s^\prime) \\
   &=\EE_{\bm{\pi}(\cdot,s^\prime)} \bigg[ \int_{s^{\prime\prime}} p(s^{\prime\prime},s^\prime,\bm{a_k}) (V_{k+1,i}^{T,\bm{\pi}}(s^{\prime\prime}) - B_{k+1}^{T,\bm{\pi}}(s^{\prime\prime})) ds^{\prime\prime} \bigg]. \nonumber
  }{
   &V_{k+1, i}^{T,\bm{\pi}}(s) - B_{k+1}^{T,\bm{\pi}}(s) = V_{k+1, i}^{T,\bm{\pi}}(s^\prime) - B_{k+1}^{T,\bm{\pi}}(s^\prime) = \\
   &\EE_{\bm{\pi}(\cdot,s^\prime)} \bigg[ \int_{s^{\prime\prime}} p(s^{\prime\prime},s^\prime,\bm{a_k}) (V_{k+1,i}^{T,\bm{\pi}}(s^{\prime\prime}) - B_{k+1}^{T,\bm{\pi}}(s^{\prime\prime})) ds^{\prime\prime} \bigg]. \nonumber
  }
 \end{align}
 where the first equality follows from the inductive assumption (i.e., \refequ{eq:ind-T-2} holds for $k+1$), and the second equality follows from applying \refequ{eq:ind-second}.
 Substituting \refequ{eq:second-ind-1} and \refequ{eq:second-ind-2} in \refequ{eq:induction}, we get:
 \[
  V_{k, i}^{T,\bm{\pi}}(s) - B_{k}^{T,\bm{\pi}}(s) = V_{k, i}^{T,\bm{\pi}}(s^\prime) - B_{k}^{T,\bm{\pi}}(s^\prime).
 \]
\end{proof}

\subsection{Infinite-horizon Case}\label{subsec:infinite-horizon-case}
So far, we have shown that, under certain assumptions, \refpro{prop:v-phi-diff} holds for the finite-horizon case. 
In this section, we extend our proof to the infinite-horizon case.
To this end, we first need to show that $\Phi(s, \bm{a})$ is bounded. 
Given \refdef{def:one-shot}, since $r_i$ is continuously differentiable (Assumption 3), $\Phi$ is also differentiable with respect to $\bm{a}$~\cite{monderer1996potential}.
Similarly, given \refcon{con:cst}, $\Phi$ is differentiable with respect to $s$, and therefore, it is continuous. 
Since the space $S \times \bm{A}$ is compact and $\Phi$ is continuous, $\Phi$ has a global maximum, and it is bounded.

Next, we present the following lemma (the proof of this lemma is deferred to the \refapp{sec:proof-lemma-1}):
\begin{lemma}
\label{lemm:lemma1}
 Let $h: S \times \bm{A} \mapsto \RR$ be a bounded function, and let $\gamma$ be a real number in $(0, 1)$.
 For any state $s$, any $0 < T < \infty$, and any strategy $\bm{\pi} \in \bm{\Pi}$, let $H^{T,\bm{\pi}}(s)$ be defined as:
 \[
  H^{T,\bm{\pi}}(s) \triangleq \EE_{\bm{\pi}} \left[ \sum_{t=0}^{T-1} \gamma^t h(s_t, \bm{a_t}) \given[\Big] s_0 = s \right].
 \]
 Then there exists a function $H:  S \times \bm{\Pi} \mapsto \RR$ such that for all states $s \in S$ and for any strategy $\bm{\pi} \in \bm{\Pi}$, we have:
 \[
  \lim_{T \to \infty} H^{T,\bm{\pi}}(s) = H^{\bm{\pi}}(s), 
 \]
 where $H^{\bm{\pi}}$ is given by:
 \[
  H^{\bm{\pi}}(s) \triangleq \EE_{\bm{\pi}} \left[ \sum_{t=0}^{\infty} \gamma^t h(s_t, \bm{a_t})  \given[\Big]  s_0 = s \right].
 \]
\end{lemma}

Given \reflmm{lemm:lemma1}, for $B^{\bm{\pi}}(s)$ and $V_i^{\bm{\pi}}(s)$ defined according to \refequ{eq:B} and \refequ{eq:value}, we have the following:
\[
 \lim_{T \to \infty} B_1^{T,\bm{\pi}}(s) = B^{\bm{\pi}}(s), \quad \text{and} \quad \lim_{T \to \infty} V_{1, i}^{T,\bm{\pi}}(s) = V_i^{\bm{\pi}}(s).
\]
Therefore, since $B^{\bm{\pi}}(s)$ and $V_i^{\bm{\pi}}(s)$ are well defined, we define $B^{\max}$ and $V_i^{\max}$ as:
\[
 B^{\max} = \max_{s,\bm{\pi}} \vert B^{\bm{\pi}}(s) \vert, \quad \text{and} \quad V_i^{\max} = \max_{s,\bm{\pi}} \vert V_i^{\bm{\pi}}(s) \vert.
\]
We are now ready to extend our proof of \refpro{prop:v-phi-diff} to the infinite-horizon case:
\begin{proof}
 We use proof by contradiction.  
 Suppose that there exists an agent $i$ and a constant $c \neq 0$ such that:
 \begin{equation}
 \label{eq:c}
  B^{\bm{\pi}}(s) - B^{\bm{\pi^\prime}}(s) = V_i^{\bm{\pi}}(s) - V_i^{\bm{\pi^\prime}}(s) + c.
 \end{equation}
 For any $0 < T^\prime < \infty$, we can write $B^{\bm{\pi}}(s)$ and $ V_i^{\bm{\pi}}(s)$ as:
 \[
  B^{\bm{\pi}}(s) = B_1^{T^\prime,\bm{\pi}}(s) + \gamma^{T^\prime} \int_{s^\prime}  B^{\bm{\pi}}(s^\prime)  \PP_{s,s^\prime}^{T^\prime,\bm{\pi}} ds^\prime,
 \]
 and 
 \[
  V_i^{\bm{\pi}}(s) = V_{1,i}^{T^\prime,\bm{\pi}}(s) + \gamma^{T^\prime} \int_{s^\prime} V_i^{\bm{\pi}}(s^\prime) \PP_{s,s^\prime}^{T^\prime,\bm{\pi}} ds^\prime,
 \]
 where $\PP_{s,s^\prime}^{k,\bm{\pi}}$ is the probability of going from state $s$ to state $s^\prime$ in $k$ steps while following joint strategy $\bm{\pi}$.
 This probability can be recursively defined for $k > 0$ as:
 \[
  \PP_{s,s^\prime}^{k,\bm{\pi}} = \int_{\bm{a}} \bm{\pi}(\bm{a} \given s) \int_{s^{\prime\prime}} p(s^{\prime\prime}, s, a) \PP_{s^{\prime\prime}, s^\prime}^{k-1, \bm{\pi}} ds^{\prime\prime} d\bm{a}.
 \]
 Here, $\PP_{s, s^\prime}^{0, \bm{\pi}}$ is 1 if $s = s^\prime$ and is 0 otherwise.
 Given the definition of $\PP_{s,s^\prime}^{k,\bm{\pi}}$, for any state $s$, strategy $\bm{\pi} \in \bm{\Pi}$, and $k \ge 0$, we have: 
 \begin{equation}
 \label{eq:sumPP}
  \int_{s^\prime} \PP_{s,s^\prime}^{k,\bm{\pi}} ds^\prime = 1.
 \end{equation}
 
 We can now write $c$ in \refequ{eq:c} as:
 \begin{align}
 \label{eq:c2}
  c &= (B^{\bm{\pi}}(s) - B^{\bm{\pi^\prime}}(s)) - (V_i^{\bm{\pi}}(s) - V_i^{\bm{\pi^\prime}}(s)) \nonumber \\
  &=(B_1^{T^\prime,\bm{\pi}}(s) - B_1^{T^\prime,\bm{\pi^{\prime}}}(s)) - (V_{1,i}^{T^\prime,\bm{\pi}}(s) - V_{1,i}{T^\prime,\bm{\pi^{\prime}}}(s)) \nonumber \\ 
  &\quad + \gamma^{T^\prime} \int_{s^\prime} (B^{\bm{\pi}}(s^\prime) - V_i^{\bm{\pi}}(s^\prime)) \PP_{s,s^\prime}^{T^\prime,\bm{\pi}}  ds^\prime \nonumber \\
  &\quad - \gamma^{T^\prime} \int_{s^\prime} (B^{\bm{\pi^\prime}}(s^\prime) - V_i^{\bm{\pi^\prime}}(s^\prime)) \PP_{s,s^\prime}^{T^\prime,\bm{\pi}} ds^\prime.
 \end{align}
 Denoting the last two terms in \refequ{eq:c2} by $C$, we have:
 \[
  c = (B_1^{T^\prime,\bm{\pi}}(s) - B_1^{T^\prime,\bm{\pi^{\prime}}}(s)) - (V_{1,i}^{T^\prime,\bm{\pi}}(s) - V_{1,i}^{T^\prime,\bm{\pi^{\prime}}}(s)) + C.
 \]
 Given \refequ{eq:sumPP}, we observe the following bound:
 \begin{equation*}
  \vert C \vert \leq 2\gamma^{T^\prime} (B^{\max} + V_i^{\max}).
 \end{equation*}
 We can choose $T^\prime$ to be sufficiently large so that we have:
 \[ 
  \gamma^{T^\prime}(B^{\max} + V_i^{\max}) < \frac{1}{4} \vert c \vert.
 \]
 This then implies:
 \[  
  \vert (B_1^{T^\prime,\bm{\pi}}(s) - B_1^{T^\prime,\bm{\pi^{\prime}}}(s)) - (V_{1,i}^{T^\prime,\bm{\pi}}(s) - V_{1,i}^{T^\prime,\bm{\pi^{\prime}}}(s)) \vert  > \frac{1}{2}c, 
 \]
 which is a contradiction because we have proved that:
 \[ 
  (B_1^{T^\prime,\bm{\pi}}(s) - B_1^{T^\prime,\bm{\pi^{\prime}}}(s)) - (V_{1,i}^{T^\prime,\bm{\pi}}(s) - V_{1,1}^{T^\prime,\bm{\pi^{\prime}}}(s)) = 0.
 \]
\end{proof}

==> Sections/6-related.tex <==
\section{Related work}\label{sec:related-work}
Monderer and Shapley introduced potential games and extensively studied their fundamental properties~\cite{monderer1996potential}.
This class of games stands as one of the most crucial and extensively studied, exemplifying multi-agent coordination, where all agents' utilities align perfectly through a potential function.
Essentially, cooperation becomes highly favorable within such games.
Notably, Monderer and Shapley proved the convergence of fictitious play to equilibrium within the class of (weighted) potential games.

Although the concept of potential games was initially defined for single-stage games, it has been extended to Markov potential games (MPGs) within the context of stochastic games.
In~\cite{leonardos2021global}, the authors established structural properties of MPGs and provided sufficient conditions for MPGs to be potential at each state.
They also proved convergence to the $\epsilon$-Nash equilibrium in MPGs with finite state space when agents independently run policy gradient on their own strategy.
Additionally, Fox et al.~\cite{fox2022independent} demonstrated that in an MPG, with all agents using independent natural policy gradient, their policies converge to the equilibrium.

In their work~\cite{macua2018learning}, the authors establish conditions regarding agents' payoff functions for a stochastic game to qualify as an MPG\@.
Additionally, they introduce two methods for deriving the potential function.
They emphasize that in a potential game scenario, finding the Nash equilibrium entails solving just one optimal control problem instead of multiple problems, each dedicated to an individual agent.
Furthermore, the study by Zhang et al.~\cite{zhang2021gradient} delves deeper into MPGs.
It offers a comprehensive discussion, encompassing examples of one-shot potential games that do not meet the MPG criteria, along with outlining sufficient conditions for a stochastic game to qualify as an MPG.
The paper also includes practical application examples, enriching the understanding of MPGs.
